Structural Parameterization of Locating-Dominating Set and Test Cover

We investigate structural parameterizations of two identification problems: LOCATING-DOMINATING SET and TEST COVER. In the first problem, an input is a graph $G$ on $n$ vertices and an integer $k$, and one asks if there is a subset $S$ of $k$ vertices such that any two distinct vertices not in $S$ are dominated by distinct subsets of $S$. In the second problem, an input is a set of items $U$, a set of subsets $\mathcal{F}$ of $U$ called $tests$ and an integer $k$, and one asks if there is a set $S$ of at most $k$ tests such that any two items belong to distinct subsets of tests of $S$. These two problems are "identification" analogues of DOMINATING SET and SET COVER, respectively. Chakraborty et al. [ISAAC 2024] proved that both the problems admit conditional double-exponential lower bounds and matching algorithms when parameterized by treewidth of the input graph. We continue this line of investigation and consider parameters larger than treewidth, like vertex cover number and feedback edge set number. We design a nontrivial dynamic programming scheme to solve TEST COVER in "slightly super-exponential" time $2^{O(|U|\log |U|)}(|U|+|\mathcal{F}|)^{O(1)}$ in the number $|U|$ of items and LOCATING-DOMINATING SET in time $2^{O(\textsf{vc} \log \textsf{vc})} \cdot n^{O(1)}$, where $\textsf{vc}$ is the vertex cover number and $n$ is the order of the graph. This shows that the lower bound results with respect to treewidth from Chakraborty et al. [ISAAC 2024] cannot be extended to vertex cover number. We also show that, parameterized by feedback edge set number, LOCATING-DOMINATING SET admits a linear kernel thereby answering an open question in [Cappelle et al., LAGOS 2021]. Finally, we show that neither LOCATING-DOMINATING SET nor TEST COVER is likely to admit a compression algorithm returning an input with a subquadratic number of bits, unless $\textsf{NP} \subseteq \textsf{coNP}/poly$.

==> fes-kernel-short.tex <==
% !TEX root = ./main.tex
%%fes-kernel-short
\section{Linear kernel for {\LD} parameterized by Feedback Edge Set Number}
\label{sec:fes-kernel-short}

We next prove Theorem~\ref{thm:LD-struct-fes}. A set of edges $X$ of a graph is a {\em feedback edge set} if $G - X$ is a forest.
The minimum size of a feedback edge set is known as the {\em feedback edge set number} ${\fes}$. %(also known as the {\em cyclomatic number}) and is denoted by ${\fes}$.
%It is well-known  that
If a graph $G$ has $n$ vertices, $m$ edges, and $r$ components, then ${\fes}(G) = m - n + r$ \cite{Diestel12}.
%%%
%

%% \begin{lemma}\label{thm:FES}
%% \LD admits a kernelization algorithm that, given an instance $(G,k)$ where $G$ has $n$ vertices, $m$ edges and feedback edge set number $\fes$, computes an equivalent instance $(G',k')$ with $\calO(\fes)$ vertices and edges, and that runs in $\calO(mn)$ time. %\ff{can it be linear i.e. $\calO(n+m)$?}
%% \end{lemma}

Our proof
%Note that the proof of Lemma~\ref{thm:FES}
is nonconstructive, in the sense that it shows the \emph{existence} of a large (but constant) number of gadget types with which the kernel can be constructed, however, as there are far too many gadgets, we cannot describe them individually. Missing parts of the proof are found in Appendix~E.
%%%
We first describe graphs of given feedback edge set number. 
%A graph $G$ with $n$ vertices, feedback edge set number $\fes$, and $c$ connected components, has exactly $n+\fes-c$ edges.
%The following is a classic description of such graphs.

\begin{proposition}[{\cite[Observation 8]{KK20}}]\label{prop:FES-structure}%see also \cite[Lemma 5.10]{ELW15}, 
Any graph $G$ with feedback edge set number $\fes$ is obtained from a multigraph $\widetilde{G}$ with at most $2\fes-2$ vertices and $3\fes-3$ edges by first subdividing edges of $\widetilde{G}$ arbitrary number of times, and then, repeatedely attaching degree~1 vertices to the graph, and $\widetilde{G}$ can be computed from $G$ in $\calO(n+\fes)$ time.
\end{proposition}

By Proposition~\ref{prop:FES-structure}, we compute the multigraph $\widetilde{G}$ in $\calO(n+ \fes)$ time, and we let $\widetilde{V}$ be the set of vertices of $\widetilde{G}$. For every edge $v_1v_2$ of $\widetilde{G}$, we have either:
\begin{enumerate}
\item $v_1v_2$ corresponds to an edge in the original graph $G$, if $v_1v_2$ has not been subdivided when obtaining $G$ from $\widetilde{G}$ (then $v_1\neq v_2$ since $G$ is loop-free), or
\item $v_1v_2$ corresponds to a component $C$ of the original graph $G$ with $\{v_1,v_2\}$ removed. Moreover, $C$ induces a tree, with two (not necessarily distinct) vertices $c_1,c_2$ in $C$, where $c_1$ is the only vertex of $C$ adjacent to $v_1$ and $c_2$ is the only vertex of $C$ adjacent to $v_2$ in $G$. (Possibly, $v_1=v_2$ and the edge $v_1v_2$ is a loop of $\widetilde{G}$.)
\end{enumerate}

To avoid dealing with the case of loops, for every component $C$ of $G\setminus\{v_1\}$ with a loop at $v_1$ in $\widetilde{G}$ and with $c_1,c_2$ defined as above, we select an arbitrary vertex $x$ of the unique path between $c_1$ and $c_2$ in $G[C]$ and add $x$ to $\widetilde{V}$. As there are at most $\fes$ loops in $\widetilde{G}$, we can assume that $\widetilde{G}$ is a loopless multigraph with at most $3\fes-2$ vertices and $4\fes-3$ edges.

%% \begin{observation}\label{obs:noloops}
%% We may assume that the multigraph $\widetilde{G}$ computed in Proposition~\ref{prop:FES-structure} has at most $3\fes-2$ vertices and $4\fes-3$ edges, and no loops.
%% \end{observation}
 
  %Every loop of $\widetilde{G}$ attached to some vertex $v$ corresponds, in $G$, to a component $C$ of $G\setminus\{v\}$ with exactly two vertices $c_1,c_2$ of $C$ adjacent to $v$, and a unique path from $c_1$ to $c_2$ in $G[C]$.

The kernelization has two steps. First, we need to handle \emph{hanging trees}, that is, parts of the graph that induce trees and are connected to the rest of the graph via a single edge. Those correspond to the iterated addition of degree 1 vertices to the graph from $\widetilde{G}$ described in Proposition~\ref{prop:FES-structure}. Step~2 will deal with the subgraphs that correspond to the edges of $\widetilde{G}$.

%\subsubsection{Handling hanging trees}
%\label{hanging-subtrees}
\subparagraph*{Step 1 -- Handling the Hanging Trees.} It is known that there is a linear-time dynamic programming algorithm to solve {\LD} on trees~\cite{SlaterTrees} (see also~\cite{ABLW20}) %for a more general algorithm for block graphs, that also solves several types of problems related to \LD).
To this end, one can in fact define the following five types of (partial) solutions. For a tree $T$ rooted at a vertex $v$, we define five types for a subset $L$ of $V(T)$ as follows:

\begin{itemize}[nolistsep]
\item Type $A$: $L$ dominates all vertices of $V(T)\setminus \{v\}$ and any two vertices of $V(T)\setminus (L\cup\{v\})$ are located.
\item Type $B$: $L$ is a dominating set of $T$ and any two vertices of $V(T)\setminus (L\cup\{v\})$ are located;
\item Type $C$: $L$ is a locating-dominating set of $T$;
\item Type $D$: $L$ is a locating-dominating set of $T$ with $v\in L$;
\item Type $E$: $L$ is a locating-dominating set of $T$ such that $v\in L$ and there is no vertex $w$ of $T$ with $N(w)\cap L=\{v\}$; 
\end{itemize}

Next, for convenience, we consider the lexicographic ordering $A<B<C<D<E$. Note that these five types of solution are increasingly constrained (so, if $X<X'$, if $L$ is a solution of type $X'$, it is also one of type $X$). %Those are the five possible behaviours of a locating-dominating set of a supergraph $G$ of $T$, in which $v$ forms a cut-vertex of $G$. 
For a tree $T$ rooted at $v$ and $X\in\{A,B,C,D,E\}$, we denote by $opt_X(T,v)$ the minimum size of a set $L\subseteq V(T)$ of type $X$. Note that $opt_C(T,v)$ is equal to the location-domination number of $T$.
%% The following proposition can be proved by using the same ideas as in the dynamic programming algorithms from \cite{ABLW20,SlaterTrees}.

\begin{proposition}
\label{prop:DP-trees}
There is a linear-time dynamic programming algorithm that, for any tree $T$ and root $v$, conjointly computes $opt_X(T,v)$ for all $X\in\{A,B,C,D,E\}$.
\end{proposition}

%\begin{proof}
%  Use the same ideas as in the dynamic programming algorithms from~\cite{ABLW20,SlaterTrees}. %\ff{Do we need to describe the DP?}
%\end{proof}

%\dm{Perhaps okay for the conference version since this is not a main result. But for journal version, strict reviewers do expect either proof or the details of similar ideas more precisely if not by a complete full proof.}

%% We next show that, for a given tree, the optimal values of solutions of different types vary by at most one.

\begin{lemma}
\label{lemma:types-bounded}
  Let $T$ be a tree with vertex $v$, and let $X,X'\in\{A,B,C,D,E\}$ with $X<X'$. We have $opt_{X'}(T,v)\leq opt_{X}(T,v)\leq opt_{X'}(T,v)+1$.%$opt_E(T,v)\leq opt_D(T,v)\leq opt_C(T,v)\leq opt_B(T,v)\leq opt_A(T,v)$. Moreover, for any $X,Y\in\{A,B,C,D,E\}$, we have $|opt_X(T,v)-opt_Y(T,v)|\leq 1$.
\end{lemma}
%% \begin{proof}
%%   The first inequality follows immediately by noticing that the conditions for types $A$ to $E$ are increasingly constrained. Moreover, all types are feasible by considering $L=V(T)$, so $opt_X(T,v)$ is always well-defined. This implies that the first inequality is true.

%%   For the second inequality, assume we have $X'\in\{A,B\}$ and $L$ is an optimal solution of type $X'$. Then, $L\cup\{v\}$ is a solution of type $E$. If $X'\in\{C,D\}$, let $L$ be an optimal solution of type $X'$. If $v\notin L$ (then $X'=C$), then again $L\cup\{v\}$ is a solution of type $E$. If $v\in L$, possibly some (unique) vertex $w$ of $T$ satisfies $N(w)\cap L=\{v\}$. Then, $L\cup\{w\}$ is a solution of type $E$. Thus, $opt_{X}(T,v)\leq opt_E(T,v)\leq opt_{X'}(T,v)+1$. In all cases, we have $opt_{X}(T,v)\leq opt_E(T,v)\leq opt_{X'}(T,v)+1$, as claimed. 
%% \end{proof}


By Lemma~\ref{lemma:types-bounded}, for any rooted tree $(T,v)$, the
five values $opt_{X}(T,v)$ (for $X\in\{A,B,C,D,E\}$) differ by at most
one, and we know that they increase along with $X$: $opt_{A}(T,v)\leq opt_{B}(T,v)\leq \ldots \leq opt_{E}(T,v)$. Hence, for any rooted tree $(T,v)$, there is one value
$X\in\{A,B,C,D,E\}$ %where the ``shift'' occurs. More precisely,
so that, whenever $X'\leq X$, we have $opt_{X'}(T,v)=opt_{X}(T,v)$, and
whenever $X'>X$, we have $opt_{X'}(T,v)=opt_{X}(T,v)+1$. Thus, we can
introduce the following definition. %%, which partitions the set of rooted
%%trees according to one of five such possible behaviours.

\begin{definition}[Rooted tree classes]
For $X\in\{A,B,C,D,E\}$, we define the class $\mathcal T_X$ as the set
of pairs $(T,v)$ such that $T$ is a tree with root $v$, and there is
an integer $k$ with $opt_{X'}(T,v)=k$ whenever $X'\leq X$, and
$opt_{X'}(T,v)=k+1$ whenever $X'>X$ (note that $k$ may differ across
the trees in $\mathcal T_X$).
\end{definition}
  %Let $G$ be a graph that can be obtained from a graph $G'$ and a tree $T$, by identifying a vertex $v$ of $T$ with a vertex $w$ of $G'$. For $X\in\{A,B,C,D,E\}$, we say that a subset $L$ of $V(G)$ is a \emph{solution of type $X$} for $G$ if $L\cap V(T)$ is of type $X$ for $(T,v)$. 
Note that for the trees in $\mathcal T_E$, all five types of optimal
solutions have the same size.
  
It is clear by Lemma~\ref{lemma:types-bounded} that the set of all possible pairs $(T,v)$ where $T$ is a tree and $v$ a vertex of $T$, can be partitioned into the five classes $\mathcal T_X$, where $X\in\{A,B,C,D,E\}$. Moreover, it is not difficult to construct small rooted trees for each of these five classes. We however omit these constructions here, since later on, we will need far more many similar gadgets, for which we cannot provide concrete examples due to their large number. See Appendix~E for the concrete constructions.

%% We next provide five such small rooted trees, each in a different class. 
%% \def\myfigscale{0.8}

%% \begin{table} \centering  
%%   \begin{tabular}{|c|c|c|c|c|c|}

%%  \hline

%%     &

%%     \scalebox{\myfigscale}{\begin{tikzpicture}[join=bevel,inner sep=0.5mm]
%%         \node (v) at (0,0) [draw, circle, label={0:$v_A$}] {}; 
%%         \node (e) at (0,-1.5) {};
%%     \end{tikzpicture}}
%%     % \hline


    
%%     &

%%     \scalebox{\myfigscale}{\begin{tikzpicture}[join=bevel,inner sep=0.5mm]
%%         \node (v) at (0,0) [draw, circle, label={0:$v_B$}] {}; 
%%         \node (a) at (0,-.5) [draw, circle] {};
%%         \node (b) at (0,-1) [draw, circle] {};
%%         \node (e) at (0,-1.5) {};
%%         \draw [-] (b)--(a)--(v);
%%     \end{tikzpicture}}
    
%%     &

%%     \scalebox{\myfigscale}{\begin{tikzpicture}[join=bevel,inner sep=0.5mm]
%%         \node (v) at (0,0) [draw, circle, label={0:$v_C$}] {}; 
%%         \node (a) at (-.25,-.5) [draw, circle] {};
%%         \node (b) at (-.5,-1) [draw, circle] {};
%%         \node (c) at (.25,-.5) [draw, circle] {};
%%         \node (d) at (.5,-1) [draw, circle] {};
%%         \node (e) at (0,-1.5) {};
%%         \draw [-] (b)--(a)--(v)--(c)--(d);
%%     \end{tikzpicture}}

   
%%     &
%%     \scalebox{\myfigscale}{\begin{tikzpicture}[join=bevel,inner sep=0.5mm]
%%         \node (v) at (0,0) [draw, circle, label={0:$v_D$}] {}; 
%%         \node (a) at (0,-.5) [draw, circle] {};
%%         \node (e) at (0,-1.5) {};
%%         \draw [-] (a)--(v);
%%     \end{tikzpicture}}

%%     &
    
%%     \scalebox{\myfigscale}{\begin{tikzpicture}[join=bevel,inner sep=0.5mm]
%%         \node (v) at (0,0) [draw, circle, label={0:$v_E$}] {}; 
%%         \node (a) at (-.25,-.5) [draw, circle] {};
%%         \node (b) at (-.5,-1) [draw, circle] {};
%%         \node (c) at (.25,-.5) [draw, circle] {};
%%         \node (d) at (.5,-1) [draw, circle] {};
%%         \node (e) at (.75,-1.5) [draw, circle] {};
%%         \draw [-] (b)--(a)--(v)--(c)--(d)--(e);% ($(v)+(-.5,0)$) -- ($(v)+(.5,0)$);
%%     \end{tikzpicture}}\\

    
%%   & $T_A$ & $T_B$  & $T_C$ & $T_D$ & $T_E$\\

%% \hline
%% $opt_A$ & 0 & 1 & 2 & 1& 3\\
%% \hline
%% $opt_B$ & 1 & 1 & 2 & 1 & 3\\
%% \hline
%% $opt_C$ & 1 & 2 & 2 & 1 & 3\\
%% \hline
%% $opt_D$ & 1 & 2 & 3 & 1 & 3\\
%% \hline
%% $opt_E$ & 1 & 2 & 3 & 2 & 3\\
%% \hline
%%   \end{tabular}
%%   \caption{The five rooted tree gadgets with their values of the five $opt_X$ functions.}
%%   \label{tab:tree-gadgets}
%% \end{table}

\begin{definition}[Rooted tree gadgets]\label{def:tree-gadgets}
For $X\in\{A,B,C,D,E\}$, let $(T_X,v_X)$ be the rooted tree of class $\mathcal T_X$ from Table~\ref{tab:tree-gadgets}, and let $k_X=opt_X(T_X,v_X)$.
\end{definition}


%As these are very small, it is easy to check that the gadgets are indeed in the claimed class. %\ff{need a proof?}

%\begin{observation}
%For $X\in\{A,B,C,D,E\}$, $(T_X,v_X)$ belongs to the class $\mathcal T_X$.
%\end{observation}

%% \begin{definition}[Simple tree gadgets]\label{def:tree-gadgets}
%% For every $X\in\{A,B,C,D,E\}$, let $(T_X,v_X)$ be the smallest rooted tree of class $\mathcal T_X$, and let $k_X=opt_X(T_X,v_X)$.
%% \end{definition}

We are now ready to present our first reduction rule.

\begin{reduction rule}
\label{reduc:hanging-tree}
Let $(G,k)$ be an instance of \LD such that $G$ can be obtained from a graph $G'$ and a tree $T$, by identifying a vertex $v$ of $T$ with a vertex $w$ of $G'$, such that $(T,v)$ is in class $\mathcal T_X$ with $X\in\{A,B,C,D,E\}$, and with $opt_X(T,v)=t$.
Then, we remove all vertices of $T\setminus\{v\}$ from $G$ (this results in $G'$), we consider $G$ and a copy of the rooted tree gadget $(T_X,v_X)$, and we identify $v_X$ with $v$, to obtain $G''$.
The reduced instance is $(G'',k-t+k_X)$.
\end{reduction rule}

\begin{lemma}\label{lemm:reduc-hanging-tree}
For an instance $(G,k)$ of \LD, Reduction Rule~\ref{reduc:hanging-tree} can be applied exhaustively in time $\calO(n^2)$, and for each application, $(G,k)$ is a YES-instance of \LD if and only if $(G'',k-t+k_X)$ is a YES-instance of \LD.
\end{lemma}

%% \begin{proof}
%%   To apply Reduction Rule~\ref{reduc:hanging-tree}, one can find all vertices of degree~1 in $G$, mark them, and iteratively mark degree~1 vertices in the subgraph induced by unmarked vertices. Note that a connected subset $S$ of marked vertices induces a tree with a single vertex $v_S$ adjacent to a non-marked vertex $w$. Moreover, at the end of the marking process, the subgraph induced by non-marked vertices has minimum degree~2. This process can be done in $\calO(n^2)$ time.% Let $v=w$.

%%   We form the set of candidate trees $T$ by taking the union $S_w$ of all marked subsets that are connected to some common unmarked vertex $w$, together with $w$. Note that all these candidate trees are vertex-disjoint. Again, this can be done in $\calO(n^2)$ time. Let $(T,v)$ be such a rooted tree, and let $G'$ be the subgraph induced by $V(G)\setminus S_v$. Then, we apply the linear-time dynamic programming algorithm of Proposition~\ref{prop:DP-trees} to $(T,v)$ to determine the class $\mathcal T_X$ to which $(T,v)$ belongs to, for some $X\in\{A,B,C,D,E\}$, as well as $opt_X(T,v)=t$ for each $X\in\{A,B,C,D,E\}$. Constructing $(G'',k-t+k_X)$ by replacing $T$ by $T_X$ in $G$ can then be done in time $\calO(|V(T)|)$. Thus, overall applying the reduction rule to all trees takes $\calO(n^2)$ time.

%%   Now, we prove the second part of the statement. Assume we have applied Reduction Rule~\ref{reduc:hanging-tree} to a single tree $(T,v)$ to $G$,that $(G,k)$ is a YES-instance of \LD, and let $L$ be an optimal locating-dominating set of $G$ of size at most $k$. Assume that $L\cap V(T)$ is of type $X'$ for $X'\in\{A,B,C,D,E\}$ with respect to $(T,v)$. Notice that the only interactions between the vertices in $V(T)$ and $V(G')$ are through the cut-vertex $v$. If $X'\leq X$, then, as $L$ is optimal, we have $|L\cap V(T)|=t$; if $X'>X$, then by Lemma~\ref{lemma:types-bounded}, we have $|L\cap V(T)|=t+1$. Now, we obtain a solution of $G''$ from $L'=L\cap V(G')$ by adding an optimal solution $S_{X'}$ of type $X'$ of $(T_X,v_X)$ to $L'$. This has size $k_X$ if $X'\leq X$ and $k_X+1$ if $X'>X$. As $S_{X'}$ behaves the same as $L\cap V(T)$ with respect to $L'$, $L$ is a valid locating-dominating set of $G''$. Its size is either $|L|-(t+1)+k_X+1$ if $X'>X$, or $|L|-t+k_X$ if $X\leq X'$, which in both cases is at most $k-t+k_X$, thus $(G'',k-t+k_X)$ is a YES-instance.

%%   The proof of the converse follows by the same argument: essentially, the trees $(T,v)$ and $(T_X,v_X)$ are interchangeable.
%% \end{proof}


%% We now use Lemma~\ref{lemm:reduc-hanging-tree} to apply Reduction Rule~\ref{reduc:hanging-tree} exhaustively in time $\calO(n^2)$, before proceeding to the second part of the algorithm.

\subparagraph*{Step 2 -- Handling the subgraphs corresponding to edges of $\widetilde{G}$.} In the second step of our algorithm, we construct tree gadgets similar to those defined in Step~1, but with \emph{two} distinguished vertices. We thus extend the above terminology to this setting. Let $(T,v_1,v_2)$, be a tree $T$ with two distinguished vertices $v_1,v_2$. We define types of trees as in the previous subsection. To do so, we first define the types for each of $v_1$ and $v_2$, and then we combine them. For $X\in\{A,B,C,D,E\}$, a subset $L$ of $V(T)$ is of \emph{type $(X,-)$ with respect to $v_1$} if: %\ff{better notation would be good}
\begin{itemize}[nolistsep]
\item Type $(A,-)$: $L$ dominates all vertices of $V(T)\setminus \{v_1,v_2\}$ and any two vertices of $V(T)\setminus (L\cup\{v_1,v_2\})$ are located.
\item Type $(B,-)$: $L$ dominates all vertices of $V(T)\setminus \{v_2\}$ and any two vertices of $V(T)\setminus (L\cup\{v_1,v_2\})$ are located;
\item Type $(C,-)$: $L$ dominates all vertices of $V(T)\setminus \{v_2\}$ and any two vertices of $V(T)\setminus (L\cup\{v_2\})$ are located;
\item Type $(D,-)$: $L$ dominates all vertices of $V(T)\setminus \{v_2\}$, $v_1\in L$, and any two vertices of $V(T)\setminus (L\cup\{v_2\})$ are located;
\item Type $(E,-)$: $L$ dominates all vertices of $V(T)\setminus \{v_2\}$, $v_1\in L$, any two vertices of $V(T)\setminus (L\cup\{v_2\})$ are located, and there is no vertex $w$ of $V(T)\setminus\{v_2\}$ with $N(w)\cap L=\{v_1\}$;
\end{itemize}

Thus, the idea for a set $L$ of type $(X,-)$ with respect to $v_1$ is that there are specific constraints for $v_1$, but no constraint for $v_2$ (and the usual domination and location constraints for the other vertices). %We also have the symmetric definitions for being of \emph{type $(-,Y)$ with respect to $v_2$}.
We say that $L$ if of type $(X,Y)$ with respect to $(T,v_1,v_2)$ if $L$ is of type $(X,-)$ with respect to $v_1$ and of type $(Y,-)$ with respect to $v_2$. Thus, we have a total of 25 such possible types. %Note that, since $v_1,v_2$ must be at distance at least~3 apart in $T$, there is no interference


We let $opt_{X,Y}(T,v_1,v_2)$ be the smallest size of a subset $L$ of $T$ of type $(X,Y)$. %Next, we argue that one can efficiently compute these values.
Here as well, there is a linear-time dynamic programming algorithm that, for any tree $T$ and two vertices $v_1,v_2$, conjointly computes $opt_{X,Y}(T,v_1,v_2)$ for all $X,Y\in\{A,B,C,D,E\}$.

%% \begin{proposition}\label{prop:DP-trees-2}
%% There is a linear-time dynamic programming algorithm that, for any tree $T$ and two vertices $v_1,v_2$, conjointly computes $opt_{X,Y}(T,v_1,v_2)$ for all $X,Y\in\{A,B,C,D,E\}$.
%% \end{proposition}

%% \begin{proof}
%% The dynamic programming is similar to that of Proposition~\ref{prop:DP-trees}. We root $T$ at $v_1$. The main difference is that extra care must be taken around $v_2$ to only keep the solutions of type $(-,Y)$ for the subtrees that contain $v_2$.%\ff{more details needed?}
%% \end{proof}


%% Next, similarly to Lemma~\ref{lemma:types-bounded}, we show that for a triple $(T,v_1,v_2)$, the optimal solution values for different types, may vary by at most~2.

\begin{lemma}\label{lemma:types-bounded-2}
  Let $T$ be a tree with vertices $v_1,v_2$ of $T$, and let $X,X',Y,Y'\in\{A,B,C,D,E\}$ with $X\leq X'$ and $Y\leq Y'$. If $X=X'$ and $Y<Y'$ or $X<X'$ and $Y=Y'$, we have $opt_{X,Y}(T,v_1,v_2)\leq opt_{X',Y'}(T,v_1,v_2)\leq opt_{X,Y}(T,v_1,v_2)+1$. If $X<X'$ and $Y<Y'$, we have $opt_{X,Y}(T,v_1,v_2)\leq opt_{X',Y'}(T,v_1,v_2)\leq opt_{X,Y}(T,v_1,v_2)+2$.
\end{lemma}
%% \begin{proof}
%%   The proof is similar to that of Lemma~\ref{lemma:types-bounded}. As before, the lower bound is clear since the conditions for type $(X',Y')$ are more constrained that those for $(X,Y)$. For the upper bound, assume first that $X=X'$ or $Y=Y'$ (without loss of generality, $Y=Y'$). Then, as before, given a solution $S$ of type $(X,Y)$, we can add to $S$ a single vertex in the closed neighbourhood of $v_1$ to obtain a solution of type $(E,Y)$. Similarly, if both $X<X'$ and $Y<Y'$, we can add to $S$ a vertex to the closed neighbourhoods of each of $v_1$ and $v_2$ and obtain a solution of type $(E,E)$.
%% \end{proof}

%% By Lemma~\ref{lemma:types-bounded-2}, we can introduce the following definition. Note that for a triple $(T,v_1,v_2)$, the minimum value of $opt_{X,Y}(T,v_1,v_2)$ over all $X,Y\in\{A,B,C,D,E\}$ is reached for $X=Y=A$ (and the maximum, for $X=Y=E$).

\begin{definition}[Doubly rooted tree classes]
  For a function $g:\{A,B,C,D,E\}^2\to\{0,1,2\}$, we define the class $\mathcal T_{g}$ as the set of triples $(T,v_1,v_2)$ such that $T$ is a tree, $v_1,v_2$ are two of its vertices, and for every $(X,Y)\in\mathcal\{A,B,C,D,E\}^2$, we have $opt_{X,Y}(T,v_1,v_2)-opt_{A,A}(T,v_1,v_2)=g(X,Y)$.
\end{definition}

There are at most $3^{25}$ possible classes of triples, since that is the number of possible functions $g$. By Lemma~\ref{lemma:types-bounded-2}, these classes define a partition of all sets of triples $(T,v_1,v_2)$. %\footnote{Some of these classes are actually empty, since, for example, by Lemma~\ref{lemma:types-bounded-2}, $opt_{X,Y}(T,v_1,v_2)$ increases with $X$ and $Y$; however, an empirical study shows that the number of nonempty classes is very large.}

We next define suitable tree gadgets for the above classes of triples. As there is a very large number of possible types of triples, we cannot give a concrete definition of such a gadget, but rather, an existential one.

\begin{definition}[Doubly-rooted tree gadgets]\label{def:double-gadget}
  For a function $g:\{A,B,C,D,E\}^2\to\{0,1,2\}$, let $(T_{g},v_X,v_Y)$ be the \emph{smallest} tree in $\mathcal T_{g}$ (if such a tree exists), and let $k_{g}=opt_{A,A}(T_{g},v_X,v_Y)$.
\end{definition}

We are now ready to present our second reduction rule, which replaces certain triples $(T,v_1,v_2)$ by gadgets from Definition~\ref{def:double-gadget}.

\begin{reduction rule}\label{reduc:hanging-tree-2}
  Let $(G,k)$ be an instance of \LD, with:
  \begin{itemize}
  \item an induced subgraph $G'$ of $G$ with two vertices $w_1,w_2$;
  \item a tree $T$ with two vertices $v_1,v_2$ with $(T,v_1,v_2)$ in class $\mathcal T_{g}$ with $g:\{A,B,C,D,E\}^2\to\{0,1,2\}$, and with $opt_{A,A}(T,v_1,v_2)=t$;
  \item $w_1,w_2$ do not belong to a hanging tree of $G$;
  \item $G$ can be obtained by taking a copy of $T$ and a copy of $G'$ and identifying, respectively, $v_1$ with $w_1$, and $v_2$ with $w_2$.
  \end{itemize}

Then, we remove all vertices of $T\setminus\{v_1,v_2\}$ from $G$ (that is, we compute $G'$), we consider $G'$ and a copy of doubly-rooted tree gadget $(T_{g},v_X,v_Y)$, and we identify $v_X$ with $v_1$ and $v_Y$ with $v_2$, to obtain $G''$. The reduced instance is $(G'',k-t+k_{g})$.
\end{reduction rule}


\begin{lemma}\label{lemm:reduc-hanging-tree-2}
For an instance $(G,k)$ of \LD, Reduction Rule~\ref{reduc:hanging-tree-2} can be applied to every tree component corresponding to an edge of $\widetilde{G}$ in time $\calO(n\fes)$, and $(G,k)$ is a YES-instance of \LD if and only if $(G'',k-t+k_{g})$ is a YES-instance of \LD.  
\end{lemma}
%% \begin{proof}
%%   To apply the reduction rule as stated, we compute the multigraph $\widetilde{G}$ in time $\calO(n+\fes)$ using Proposition~\ref{prop:FES-structure}; by Observation~\ref{obs:noloops}, we can assume it has no loops and at most $4\fes-3$ edges. Now, for every edge $xy$ of $\widetilde{G}$, we select the neighbour $v_1$ of $x$ and the neighbour $v_2$ of $y$ in $G$, that lie on the $xy$-path corresponding to the edge $xy$ of $\widetilde{G}$. The tree $(T,v_1,v_2)$ is the subgraph of $G$ corresponding to the edge $xy$ of $\widetilde{G}$, and $G'$ is the subgraph of $G$ obtained by removing $T\setminus\{v_1,v_2\}$ from $G$. Computing all these subgraphs can be done in time $\calO(n\fes)$. Computing the type $\mathcal{T}_g$ of $(T,v_1,v_2)$ can be done in time $\calO(|T|)$ by Proposition~\ref{prop:DP-trees-2}, so overall, the running time of this step is $\calO(n\fes)$.

%%   Note that all the computed subgraphs are vertex-disjoint, we can thus now apply Reduction Rule~\ref{reduc:hanging-tree-2} in time $\calO(|T|)$ to each tree $T$, noting that the gadget $T_g$ is of constant size.
  
%% For the second part of the statement, the arguments are the same as those of Lemma~\ref{lemm:reduc-hanging-tree}: since they belong to the same class $\mathcal T_{g}$, the trees $(T,v_1,v_2)$ and $(T_{g},v_X,v_Y)$ have the same behaviour with respect to \LD and the overall solution for the graph.
%% \end{proof}


\subparagraph*{Completion of the proof.} By Lemma~\ref{lemm:reduc-hanging-tree} and Lemma~\ref{lemm:reduc-hanging-tree-2}, we can apply Reduction Rule~\ref{reduc:hanging-tree} and Reduction Rule~\ref{reduc:hanging-tree-2} in time $\calO(n^2+n\fes)=\calO(mn)$. Since $\widetilde{G}$ has at most $3\fes-2$ vertices and $4\fes-3$ edges, we replaced each vertex of $\widetilde{G}$ by a constant-size tree-gadget from Definition~\ref{def:tree-gadgets} and each edge of $\widetilde{G}$ by a constant-size doubly-rooted tree gadget from Definition~\ref{def:double-gadget}, the resulting graph has $\calO(\fes)$ vertices and edges.% , as claimed. The running time is $2^{\calO(\fes)} + n^{\calO(1)}$ by first computing the kernel and then solving \LD\ in time $2^{\calO(n)}=2^{\calO(\fes)}$ on that kernel. This completes the proof of Lemma~\ref{thm:FES}.

























%% \newpage


%% Let $X$ be a minimum feedback edge set of $G$.
%% Then, $|X| = {\fes}(G)$, the value ${\fes}(G)$ is the {\em feedback edge set number} of $G$, and
%%  $G - X$ is a forest.
%% It follows from \cite{Diestel12} that if a graph $G$ has $r$ connected components, $n$ vertices, and $m$ edges, then ${\fes}(G) = m - n + r$.
%% Due to lack of space, in this section, we provide a short proof sketch of a kernel for {\LD} with $\calO({\fes})$ vertices (detailed proof can be found in appendix).
%% This proof is nonconstructive, i.e. we prove the existence of a large (but constant) number of gadget types that can be constructed.
%% But the number of gadget types is so large that we do not describe them individually.
%% It is also well-known due to Kellerhels and Koana \cite{KK20} that any graph $G$ with feedback edge set number ${\fes}$ can be computed from a multigraph $\widetilde{G}$ with at most $2{\fes} - 2$ vertices and $3{\fes} - 3$ edges in $\calO(n + {\fes})$-time.
%% In particular, using the ideas of this algorithm of \cite{KK20}, we can also compute the corresponding multigraph $\widetilde{G}$ from $G$ in polynomial-time.
%% We describe a short proof sketch of Theorem \ref{thm:LD-struct-fes} for the rest of the section.
 
%% \subparagraph*{Proof Sketch of Theorem \ref{thm:LD-struct-fes}}
%%  Our kernelization algorithm has two phases.
%% The first phase is {handling the hanging trees}, i.e. the parts of the graph that induce trees and are connected to the rest of the graph via a single edge.
%% The second phase is {handling the subgraphs} that correspond to the edges of $\widetilde{G}$.

%% \subparagraph*{Phase 1 -- Handling Hanging Trees}
%% In this phase, we solve several types of {\LD} related problems in each of the hanging trees.
%% If $T$ is a hanging tree rooted at $v$, we define five types for a subset $L$ of $V(T)$.
%% We say that $L$ is a locating dominating set of {\bf (i)} {\em Type-$A$} if $L$ dominates all vertices of $V(T) \setminus \{v\}$ and any two vertices of $V(T) \setminus (L \cup \{v\})$ are located, {\bf (ii)} {\em Type-$B$} and any two vertices of $V(T) \setminus (L \cup \{v\})$ are located, {\bf (iii)} {\em Type-$C$} if $L$ is a locating dominating set of $T$, {\bf (iv)} {\em Type-$D$} if $L$ is a locating dominating set of $T$ with $v \in L$, and {\bf (v)} {\em Type-$E$} if $L$ is a locating dominating set of $T$ such that $v \in L$ and there is no vertex $w \in T$ with $N(w) \cap L = \{v\}$.
%% For a tree $T$ rooted at $v$ and $X \in \{A, B, C, D, E\}$, we use $opt_X(T, v)$ to denote the minimum size of a locating dominating set of $T$ of type $X$.
%% Clearly, $opt_C(T, v)$ denotes the minimum size of a locating dominating set of $T$.
%% In the next step, we define ${\calT}_X$ {\em rooted tree class} for $X \in \{A, B, C, D, E\}$, as the set of pairs $(T, v)$ such that $T$ is a tree rooted at $v$ and there is an integer $k$ with $opt_{X}(T, v) = k$.

%% \subparagraph*{Handling the Subgraphs Corresponding to the Edges of $\widetilde{G}$.}


